A coronagraphic search for wide sub-stellar companions among members of the Ursa Major moving group

We present the results of a survey to detect low-mass companions of UMa group members, carried out in 2003-2006 with NACO at the ESO VLT. While many extra-solar planets and planetary candidates have been found in close orbits around stars by the radial velocity and the transit method, direct detections at wider orbits are rare. The Ursa Major (UMa) group, a young stellar association at an age of about 200-600 Myr and an average distance of 25 pc, has not yet been addressed as a whole although its members represent a very interesting sample to search for and characterize sub-stellar companions by direct imaging. Our goal was to find or to provide detection limits on wide sub-stellar companions around nearby UMa group members using high-resolution imaging. We searched for faint companions around 20 UMa group members within 30 pc. The primaries were placed below a semi-transparent coronagraph, a rather rarely used mode of NACO, to increase the dynamic range of the images. In most cases, second epoch images of companion candidates were taken to check whether they share common proper motion with the primary. Our coronagraphic images rule out sub-stellar companions around the stars of the sample. A dynamical range of typically 13-15 mag in the Ks band was achieved at separations beyond 3" from the star. Candidates as faint as Ks ~ 20 were securely identified and measured. The survey is most sensitive between separations of 100 and 200 au but only on average because of the very different target distance. Field coverage reaches about 650 au for the most distant targets. Most of the 200 candidates are visible in two epochs. All of those were rejected being distant background objects.

==> tables/det_limits.tex <==
         HD 11131   &2004-07-22& 720&   39.0&   20.3&   11.9&14.1&   86.7&12.3&   50.7& 9.8&   22.3\\                                                                                                                                 
         HD 11171   &2004-07-27& 495&   50.4&   24.9&   12.6&15.4&  182.1&13.6&   63.9&11.1&   29.3\\                                                                                                                                 
         HD 11171   &2006-08-03&1680&   50.4&   30.1&   13.9&15.4&  247.7&13.6&   75.5&11.1&   32.9\\                                                                                                                                 
    HD 22049$^1$    &2004-09-03&2475&    8.5&    7.3&    ---&13.2&    8.7&11.3&    5.0& 8.9&    2.6\\                                                                                                                                 
         HD 22049   &2005-12-23& 720&    9.9&    8.3&    ---&13.2&   10.7&11.3&    7.2& 8.9&    0.7\\                                                                                                                                 
         HD 26913   &2003-12-25& 864&   32.8&   18.1&   16.5&13.7&  515.8&11.9&   40.4& 9.4&   18.6\\                                                                                                                                 
         HD 26913   &2005-12-06& 630&   32.3&   19.0&   12.0&13.7&   97.0&11.9&   45.5& 9.4&   18.0\\                                                                                                                                 
         HD 26923   &2003-12-26& 630&   35.8&   20.3&   18.4&14.1&    ---&12.3&   52.1& 9.8&   20.7\\                                                                                                                                 
    HD 38393$^2$    &2003-12-01&1673&   25.3&   13.4&   11.9&14.7&   96.4&12.8&   31.1&10.4&   10.6\\                                                                                                                                 
    HD 41593$^3$    &2003-12-17&1260&   25.1&   12.2&   11.8&13.5&   60.9&11.7&   30.2& 9.2&   14.7\\                                                                                                                                 
         HD 41593   &2005-11-08& 630&   24.7&   12.2&   11.5&13.5&   53.8&11.7&   30.1& 9.2&   12.6\\                                                                                                                                 
    HD 60491$^4$    &2003-12-26&1855&   43.6&   18.7&   15.8&13.4&    ---&11.5&   45.7& 9.1&   24.5\\                                                                                                                                 
         HD 60491   &2005-11-08& 560&   33.7&   19.8&   12.5&13.4&    ---&11.5&   48.8& 9.1&   18.8\\                                                                                                                                 
         HD 61606   &2004-01-10& 560&   23.2&   12.5&   12.2&13.3&  345.3&11.4&   25.6& 9.0&   12.2\\                                                                                                                                 
         HD 61606   &2005-11-08& 630&   22.9&   11.7&   11.1&13.3&   45.6&11.4&   26.4& 9.0&   10.5\\                                                                                                                                 
         HD 63433   &2004-01-15& 980&   39.8&   19.3&   14.0&13.8&    ---&12.0&   46.5& 9.5&   23.2\\                                                                                                                                 
        HIP 57548   &2004-01-11& 630&    8.1&    8.1&    ---& 9.4&    2.9& 7.5&    0.7& 5.1&    ---\\                                                                                                                                 
         HD 95650   &2004-01-14& 630&   16.3&   11.7&   11.6&12.1&   30.9&10.2&   13.7& 7.8&    8.6\\                                                                                                                                 
        HD 125451   &2004-01-29& 630&   58.6&   29.4&   19.5&15.1&    ---&13.2&   91.0&10.8&   35.8\\                                                                                                                                 
   HD 135599$^5$    &2004-07-13&1080&   22.1&   11.4&   10.9&13.4&   43.0&11.6&   22.8& 9.1&   11.9\\                                                                                                                                 
        HD 135599   &2006-04-06&1680&   24.6&   12.0&   10.8&13.4&   49.8&11.6&   32.2& 9.1&   11.6\\                                                                                                                                 
        HD 139006   &2004-02-10& 620&  102.9&   38.5&   26.5&17.0&    ---&15.2&    ---&12.7&   60.4\\                                                                                                                                 
        HD 147584   &2004-02-10& 665&   23.2&   12.5&   12.3&14.2&    ---&12.3&   25.3& 9.9&   12.4\\                                                                                                                                 
        HD 147584   &2006-02-21& 630&   26.5&   11.9&   11.1&14.2&   47.4&12.3&   32.7& 9.9&   12.0\\                                                                                                                                 
   HD 165185$^6$    &2004-08-06& 810&   30.4&   12.5&   11.2&14.1&   54.6&12.3&   36.2& 9.8&   16.8\\                                                                                                                                 
        HD 165185   &2006-06-27&1680&   32.4&   18.6&   11.3&14.1&   65.5&12.3&   47.4& 9.8&   17.2\\                                                                                                                                 
        HD 175742   &2004-07-30& 540&   30.7&   15.7&   11.9&13.4&   77.5&11.6&   33.1& 9.1&   17.7\\                                                                                                                                 
        HD 175742   &2006-06-27&1680&   30.6&   18.6&   11.4&13.4&   70.0&11.6&   44.8& 9.1&   16.8\\                                                                                                                                 
   HD 217813$^7$    &2003-10-06&1146&   43.3&   21.6&   18.0&14.2&    ---&12.3&   60.1& 9.9&   25.0\\                                                                                                                                 
       HIP 104383   &2003-11-07& 630&   33.5&   17.0&   14.3&13.1&    ---&11.3&   35.5& 8.8&   18.5\\                                                                                                                                 


==> tables/multiples.tex <==
                                      HD 11131     &1.00000&183.8000&250.0& HD 11171   & vis binary         \\
                                      HD 11171     &1.52000&        &     &            &                    \\
                                      HD 22049     &0.79000&        &     &            &                    \\
                                      HD 22049 b   &0.00140&  1.0530&     & HD 22049   & RV planet          \\
                                      HD 24916 A   &0.70000&        &     &            & vis binary         \\
                                      HD 24916 B   &0.30000& 11.0000& 17.0& HD 24916 A & vis binary         \\
                                      HD 26913     &0.96000& 65.5000&315.0& HD 26923   &                    \\
                                      HD 26923     &1.07000&        &     &            & quadruple          \\
                                      HD 26923 C   &0.60000&215.7000& 47.0& HD 26923   &                    \\
                                      HD 26923 D   &0.60000& 52.7000&139.0& HD 26923 C &                    \\
                                      HD 29875 A   &1.50000&        &     &            & vis binary         \\
                                      HD 29875 B   &0.35000&  6.6000&121.0& HD 29875 A & vis binary         \\
                                      HD 38393 A   &1.23000&        &     &            & vis triple         \\
                                      HD 38393 B   &0.80000& 94.0000&350.0& HD 38393 A & vis triple         \\
                                      HD 38393 C   &0.30000& 45.0000&345.0& HD 38393 B &                    \\
                                      HD 41593     &0.89000&        &     &            & single             \\
                                      HD 60491     &       &        &     &            &              single\\
                                      HD 61606 A   &0.81000&        &     &            & vis binary         \\
                                      HD 61606 B   &0.62000& 57.9000&112.0& HD 61606 A & single             \\
                                      HD 63433     &0.99000&        &     &            &              single\\
                                      HD 95650     &       &        &     &            &              single\\
                                      HD 98712 A   &0.75000&        &     &            & vis binary         \\
                                      HD 98712 B   &0.50000&  6.3000&307.0& HD 98712 A & vis binary         \\
                                      HIP 57548    &       &        &     &            &              single\\
                                      HD 125451 A  &1.40000&        &     &            & vis                \\
                                      HD 125451 B  &0.75000&154.4000&217.0& HD 125451 A& vis                \\
                                      GJ 569 A     &0.35000&        &     &            & no RV              \\
                                      GJ 569 B     &0.12500&  5.0000&     & GJ 569 A   & vis                \\
                                      GJ 569 Ba    &0.10500&        &     &            & binary             \\
                                      GJ 569 Bb    &0.02000&  0.0940&     & GJ 569 Ba  & vis                \\
                                      HD 134083 A  &1.33000&        &     &            & vis                \\
                                      HD 134083 B  &0.50000&108.2000& 55.0& HD 134083 A& vis                \\
                                      HD 134083 C  &0.60000&252.3000& 50.0& HD 134083 A&                    \\
                                      HD 134083 C  &0.60000&141.7000& 37.0& HD 134083 B&                    \\
                                      HD 135599    &0.85000&        &     &            &              single\\
                                      HD 139006    &2.31000&        &     &            & ecl. binary        \\
                                      HD 147584 A  &1.14000&        &     &            & SB1                \\
                                      HD 147584 B  &0.27000&  0.0090&     & HD 147584 A& RV                 \\
                                      HD 165185    &       &        &     &            & single             \\
                                      HD 175742 A  &0.75000&        &     &            & SB1                \\
                                      HD 175742 B  &0.35000&  0.0010&     & HD 175742 A& RV                 \\
                                      HIP 104383 A &0.70000&        &     &            & speckle binary     \\
                                      HIP 104383 B &0.50000&  0.3020&287.0& HIP 104383 & vis                \\
                                      HIP 104383 C &0.30000& 25.0000&     & HIP 104383 & vis                \\
                                      HD 217813    &1.05000&        &     &      single&                    \\

